Program Translation via Code Distillation

Software version migration and program translation are an important and costly part of the lifecycle of large codebases. Traditional machine translation relies on parallel corpora for supervised translation, which is not feasible for program translation due to a dearth of aligned data. Recent unsupervised neural machine translation techniques have overcome data limitations by included techniques such as back translation and low level compiler intermediate representations (IR). These methods face significant challenges due to the noise in code snippet alignment and the diversity of IRs respectively. In this paper we propose a novel model called Code Distillation (CoDist) whereby we capture the semantic and structural equivalence of code in a language agnostic intermediate representation. Distilled code serves as a translation pivot for any programming language, leading by construction to parallel corpora which scale to all available source code by simply applying the distillation compiler. We demonstrate that our approach achieves state-of-the-art performance on CodeXGLUE and TransCoder GeeksForGeeks translation benchmarks, with an average absolute increase of 12.7% on the TransCoder GeeksforGeeks translation benchmark compare to TransCoder-ST.

==> figs/compare_LLVM_IR_with_Distilling_Code.tex <==
% https://www.overleaf.com/learn/latex/Code_Highlighting_with_minted
\begin{figure*}[!ht]
\centering

\begin{adjustbox}{width=\linewidth}
\begin{tabular}{ccc}
Code & LLVM IR & Distilled Code \\
\hline \\[3mm]

\begin{minipage}{\linewidth/3}
\begin{minted}[escapeinside=||,fontsize=\small]{cpp}

    int foo(int a, int b){
      if (a<0 && b<0){
        return 0;
        }
      return pow(a,b);
    }
\end{minted}
\end{minipage} &

\begin{minipage}{\linewidth/3}
\begin{minted}[escapeinside=||,fontsize=\scriptsize]{llvm}

define dso_local 
i32 @"foo"(i32 %0, i32 %1) 
local_unnamed_addr #3 {
  %3 = and i32 %1, %0
  %4 = icmp slt i32 %3, 0
  br i1 %4, label %10, label %5
5: %preds = %2
  %6 = sitofp i32 %0 to double
  %7 = sitofp i32 %1 to double
  %8 = tail call double 
  @pow(double %6, double %7) #6
  %9 = fptosi double %8 to i32
  br label %10
10: %preds = %2, %5
  %11 = phi i32 [%9, %5], [0, %2]
  ret i32 %11
}
\end{minted} 
\end{minipage} &

\begin{minipage}{\linewidth/3}
\begin{minted}[escapeinside=||,fontsize=\small]{java}

    foo(a, b) {
      if (a<0 && b<0) {
        return 0;
      }
      return pow(a,b);
    }
\end{minted} 
\end{minipage} \\[3cm]

\begin{minipage}{\linewidth/3}
\begin{minted}[escapeinside=||,fontsize=\small]{python}

    def foo(a, b):
      if (a<0 and b<0):
        return 0
      return a**b
  
\end{minted}
\end{minipage} &

\begin{minipage}{\linewidth/3}
\begin{minted}[escapeinside=||,fontsize=\scriptsize]{llvm}

define 
i32 @"foo"(i32 %argc, i32 %argv) 
local_unnamed_addr personality 
@seq_personality {
entry:
  tail call void @seq_init(i32 4)
  %0 = tail call @seq_alloc(i64 2320)
  %1 = getelementptr %0, i64 290
  %2 = tail call {} 
  @seq_gc_add_roots(%0, %1)
  tail call fastcc void 
  @"__internal__.
  class_populate_vtables
  :0[Ptr[Ptr[Ptr[byte]]]].513"(%0)
  ret i32 0
}
\end{minted} 
\end{minipage} &

\begin{minipage}{\linewidth/3}
\begin{minted}[escapeinside=||,fontsize=\small]{java}

    foo(a, b) {
      if (a<0 && b<0) {
        return 0;
      }
      return pow(a,b);
    }
\end{minted} 
\end{minipage} \\


\end{tabular}
\end{adjustbox}

\caption{\small{\textbf{Comepare LLVM IR to our distilled code} We use a pair of parallel program cases (C++ in the first column, Python in the second column) to compare our proposed approach, distilled code and LLVM IR. Note that due to variations in the compiler front-ends used by different programming languages, the IR generated by them may also vary significantly. Our results show that distilled code displays a higher level of conciseness, elegance, and readability compared to LLVM IR.}}
\label{fig:compare_LLVM_IR_with_Distilling_Code}

\end{figure*}


==> figs/withdraw_of_transcoder_transcoder-st.tex <==
\begin{figure}[!ht]
\centering

\begin{adjustbox}{width=\linewidth}
\begin{tabular}{p{3cm} | p{10cm}}
\midrule
\textbf{Input function} &
\begin{minipage}{\textwidth}
\begin{minted}[escapeinside=||,fontsize=\meddile]{java}
// Java
static boolean isPrime(int p) {
  double checkNumber=Math.pow(2,p)-1;
  double nextval=4%checkNumber;
  for (int i=1; i<p-1; i++) {
    nextval=(nextval*nextval-2)%checkNumber;
  }
  return (nextval==0);
}
\end{minted}
\end{minipage} \\


\midrule
\textbf{TransCoder} &
\begin{minipage}{\textwidth}
\begin{minted}[escapeinside=||,fontsize=\meddile]{cpp}
// Cpp
bool isPrime(int p) {
  double checkNumber=Math.pow(2,p)-1;
  double nextval=4%checkNumber;
  for (int i=1; i<p-1; i++) {
    nextval=(nextval*nextval-2)%checkNumber;
  }
  return (nextval==0);
}
\end{minted}
\end{minipage}\\

\bottomrule
\end{tabular}
\end{adjustbox}

\caption{\small{\textbf{The drawback of TransCoder} This code snippet implements a test for primality using the Lucas-Lehmer series. The use of the modulus operator ("\%") on a double value in the C++ programming language is not considered a legal operation. This fact is not captured by the transcoder, leading to the translated code not executing properly.}}
\label{fig:withdraw_of_transcoder_transcoder-st}

\end{figure}

